Holographic Algorithms with Matchgates Capture Precisely Tractable Planar #CSP

Valiant introduced matchgate computation and holographic algorithms. A number of seemingly exponential time problems can be solved by this novel algorithmic paradigm in polynomial time. We show that, in a very strong sense, matchgate computations and holographic algorithms based on them provide a universal methodology to a broad class of counting problems studied in statistical physics community for decades. They capture precisely those problems which are #P-hard on general graphs but computable in polynomial time on planar graphs. More precisely, we prove complexity dichotomy theorems in the framework of counting CSP problems. The local constraint functions take Boolean inputs, and can be arbitrary real-valued symmetric functions. We prove that, every problem in this class belongs to precisely three categories: (1) those which are tractable (i.e., polynomial time computable) on general graphs, or (2) those which are \#P-hard on general graphs but ractable on planar graphs, or (3) those which are #P-hard even on planar graphs. The classification criteria are explicit. Moreover, problems in category (2) are tractable on planar graphs precisely by holographic algorithms with matchgates.

==> X-proof.tex <==
\section{Proof Details for Theorem \ref{thm:a010b}}

Here we prove that for any $c \not = 1$, we can assign
suitable complex values to $x,y$ and $t$, where $t \not =0$, 
such that $A = B = C \not = 0$, and $D=0$,
where
\begin{eqnarray*}
A &=& x^4 y^4 t+t+4 x^3 y^2+4 x+4 x^2 y+\frac{2 c x^2}{t}\\
B &=& 2 y^2 t+12 y+\frac{2c}{t} \\
C &=& 2 x y^2 t+4 x^2 y^2+4+4 x y+\frac{2 c x}{t}\\
D &=&x^2 y^3 t+y t+3 x^2 y^2+3+6 x y+\frac{2 c x}{t}.
\end{eqnarray*}


\begin{lemma}
For any $c \not = 1$, 
\[(x-1)^2 = \frac{16}{c-1}\]
has a solution $x  \not \in \{0, +1, -1\} $.
This $x$ satisfies
\begin{equation}\label{lm-1-eqn1}
\left( 2 - \frac{x(x+3)}{x-1} \right) 
\left(  \frac{x+3}{x-1} \right)
+ cx + 6 =0 \textrm{.}
\end{equation}
\end{lemma}

\begin{proof} 
Clearly $x=1$ is not a solution to $(x-1)^2 = \frac{16}{c-1}$.
Also the equation  has two distinct roots.
When $c=17$ there is a solution $x=2 \not \in \{0, +1, -1\} $.
When $c \not = 17$, we can verify $x=0$ is not a solution.
Hence the equation always has a solution other than $0, \pm 1$.

To verify (\ref{lm-1-eqn1})
we have
\begin{eqnarray*}
& & (2x -2 - x^2 -3x)(x+3) + (cx +6)(x^2 -2x +1)\\
&=& -(x^3 + 4x^2 + 5x + 6) + c x^3 + (6-2c) x^2 +(-12 +c) x + 6 \\
&=& (c-1) x^3 - 2 (c-1) x^2 + (c-17) x\\
&=& (c-1) x [ (x-1)^2 -{16}/(c-1) ]\\
&=& 0.
\end{eqnarray*}


\end{proof}

Now we fix $x  \not \in \{0, +1, -1\} $ satisfying (\ref{lm-1-eqn1})
for any given $c \not = 1$.

\begin{lemma}
For any $c \not = 1$, we can pick $z \not = \pm 1$ such that
\begin{equation}\label{lm-2-eqn1}
\frac{4 z}{(1+z)^2} = \frac{ x(x+3)}{x-1}.
\end{equation}
\end{lemma}

\begin{proof} We are given  $x \not = 0, \pm 1$.
If $x=-3$, we can pick $z =0$.
Now suppose $x \not =-3$.  Consider the quadratic
equation in $z$
\[4 z (x-1) = x (x+3) (1+z)^2.\]
This is quadratic since $x (x+3) \not =0$.
We can check that $z= + 1$ (and $-1$ respectively) is not a solution,
as this would force $x = - 1$ (and $+1$ respectively).
However, any solution where  $z \not = -1$ and $x \not = 1$
is equivalent to (\ref{lm-2-eqn1}).
Hence we have a solution $z \not = \pm 1$ to (\ref{lm-2-eqn1}).

\end{proof}

Now we further fix a  $z \not = \pm 1$ 
satisfying (\ref{lm-2-eqn1}), and let $y = z/x$ such that $xy \not = \pm 1$,
for any $c \not = 1$.


\begin{lemma}
For any  $c \not = 1$, there exist $x \not \in \{0, +1, -1\} $
and $y$ such that $xy \not = \pm 1$ satisfying
\begin{equation}\label{lm-3-eqn2}
%4y (x-1)  =  (x+3)(1+xy)^2 \\ \label{lm-3-eqn1}
\frac{2 (1 + x^2 y^2)}{(1+ xy)^2} \cdot \frac{x+3}{x-1}
+ cx + 6 = 0.
%+ cx + 6 = 0  \label{lm-3-eqn2}
\end{equation}
\end{lemma}


\begin{proof} 
%Equation (\ref{lm-3-eqn1}) is proved in (\ref{lm-2-eqn1}).
%
%For (\ref{lm-3-eqn2}) we verify
\begin{eqnarray*}
& & \frac{2 (1 + x^2 y^2)}{(1+ xy)^2} \cdot \frac{x+3}{x-1}
+ cx + 6 \\
& = & 2 \left( 1 - \frac{2z}{(1+ z)^2} \right) \cdot \frac{x+3}{x-1}
+ cx + 6 \\
& = & \left( 2 - \frac{x (x+3)}{x-1} \right) \cdot \frac{x+3}{x-1}
+ cx + 6 \\
& = & 0.
\end{eqnarray*}
Here we used (\ref{lm-2-eqn1}) and (\ref{lm-1-eqn1}).

\end{proof}


Now we will set $t = 4/(1+xy)^2$.  Clearly $t \not =0$.
We next verify that $D = 0$.

%By (\ref{lm-3-eqn1}) and (\ref{lm-3-eqn2}) we get
By (\ref{lm-2-eqn1}) and (\ref{lm-3-eqn2}) we get
\[\frac{8 y (1 + x^2 y^2)}{(1+ xy)^4} + cx + 6 = 0.\]
Then
\[t^2 y (1 + x^2 y^2) + 2 c x +  3t (1+ xy)^2 =0.\]
Thus
\[D = yt (1 + x^2 y^2) + 3  (1+ xy)^2 + \frac{2 c x}{t} = 0.\]

Next we show that $C = \frac{4 (1-xy)^2}{1-x} \not =0$.

By $D=0$, we have 
\[
C = 2 x y^2 \frac{4}{(1+ xy)^2} + 4 (1+ xy)^2 - 4 xy + 
[- yt (1 + x^2 y^2) - 3 (1+ xy)^2].
\]
Hence
\begin{eqnarray*}
C &=& \frac{8xy^2}{(1+ xy)^2} + (1+ xy)^2 - 4 xy 
- y \frac{4 (1 + x^2 y^2)}{(1+ xy)^2}\\
 &=& \frac{4y}{(1+ xy)^2} \left[ 2xy - 1 - x^2 y^2 \right]
+ (1-xy)^2 \\
 &=& \left( \frac{-4y}{(1+ xy)^2} + 1 \right) (1-xy)^2 \\
 %&=& \left( - {x+3}/(x-1) + 1)...
 &=& \frac{4 (1-xy)^2}{1-x} \not = 0,
\end{eqnarray*}
using (\ref{lm-2-eqn1}).

The next task is to show $B=C$.

We have
\[ C = 4 (1-xy)^2 + x B.\]
Hence
\[ B= \frac{1}{x}
\left[  \frac{4 (1-xy)^2}{1-x} -  4 (1-xy)^2 \right]
= \frac{4 (1-xy)^2}{x} \left[ \frac{1}{1-x} -1 \right] 
= \frac{4 (1-xy)^2}{1-x}
=C.\]
%
Finally we verify $A=C$ as well.
%
\[A = (x^4 y^4 +1) t + x [ C - 2 x y^2 t ]
= C + (x-1)C - 2 x^2 y^2 t + (x^4 y^4 +1) t
= C - 4 (1-xy)^2 + t (x^2 y^2-1)^2
%=C  - 4 (1-xy)^2 + t (xy+1)^2 (1-xy)^2
= C.\]








==> hisX-proof.tex <==
\section{Proof Details for Theorem \ref{thm:a010b}}

Here we prove that for any $c \not = 1$, we can assign
suitable complex values to $x,y$ and $t$, where $t \not =0$,
such that $A = B = C \not = 0$, and $D=0$,
where
\begin{eqnarray*}
A &=& x^4 y^4 t+t+4 x^3 y^2+4 x+4 x^2 y+\frac{2 c x^2}{t}\\
B &=& 2 y^2 t+12 y+\frac{2c}{t} \\
C &=& 2 x y^2 t+4 x^2 y^2+4+4 x y+\frac{2 c x}{t}\\
D &=&x^2 y^3 t+y t+3 x^2 y^2+3+6 x y+\frac{2 c x}{t}
\end{eqnarray*}


\begin{lemma}
For any $c \not = 1$,
\[(x-1)^2 = \frac{16}{c-1}\]
has a solution $x  \not \in \{0, +1, -1\} $.
This $x$ satisfies
\begin{equation}\label{lm-1-eqn1}
\left( 2 - \frac{x(x+3)}{x-1} \right) \left(  \frac{x+3}{x-1}
\right) + cx + 6 =0 \textrm{.}
\end{equation}
\end{lemma}

\begin{proof} Clearly $x=1$ is not a solution to $(x-1)^2 =
\frac{16}{c-1}$. Also the equation  has two distinct roots. When
$c=17$ there is a solution $x=2 \not \in \{0, +1, -1\} $. When $c
\not = 17$, we can verify $x=0$ is not a solution. Hence the
equation always has a solution other than $0, \pm 1$.

To verify (\ref{lm-1-eqn1})
we have
\begin{eqnarray*}
& & (2x -2 - x^2 -3x)(x+3) + (cx +6)(x^2 -2x +1)\\
&=& -(x^3 + 4x^2 + 5x + 6) + c x^3 + (6-2c) x^2 +(-12 +c) x + 6 \\
&=& (c-1) x^3 - 2 (c-1) x^2 + (c-17) x\\
&=& (c-1) x [ (x-1)^2 - \frac{16}{c-1} ]\\
&=& 0.
\end{eqnarray*}


\qed
\end{proof}

Now we fix $x  \not \in \{0, +1, -1\} $ satisfying (\ref{lm-1-eqn1})
for any given $c \not = 1$.

\begin{lemma}
For any $c \not = 1$, we can pick $z \not = \pm 1$ such that
\begin{equation}\label{lm-2-eqn1}
\frac{4 z}{(1+z)^2} = \frac{ x(x+3)}{x-1}.
\end{equation}
\end{lemma}

\begin{proof} We are given  $x \not = 0, \pm 1$. If $x=-3$, we can pick
$z =0$. Now suppose $x \not =-3$.  Consider the quadratic equation
in $z$
\[4 z (x-1) = x (x+3) (1+z)^2.\]
This is quadratic since $x (x+3) \not =0$.
We can check that $z= + 1$ (and $-1$ respectively) is not a solution,
as this would force $x = - 1$ (and $+1$ respectively).
However, any solution where  $z \not = -1$ and $x \not = 1$
is equivalent to (\ref{lm-2-eqn1}).
Hence we have a solution $z \not = \pm 1$ to (\ref{lm-2-eqn1}).


\end{proof}

Now we further fix a $y = z/x$ such that $xy \not = \pm 1$
for any $c \not = 1$.


\begin{lemma}
For any  $c \not = 1$, there exist $x \not \in \{0, +1, -1\} $
and $y$ such that $xy \not = \pm 1$ such that
\begin{equation}
4y (x-1)  =  (x+3)(1+xy)^2 \label{lm-3-eqn1}
\end{equation}
\begin{equation}
\frac{2 (1 + x^2 y^2)}{(1+ xy)^2} \cdot \frac{x+3}{x-1}
+ cx + 6 = 0  \label{lm-3-eqn2}
\end{equation}
\end{lemma}


\begin{proof} Equation (\ref{lm-3-eqn1}) is proved in
(\ref{lm-2-eqn1}).

For (\ref{lm-3-eqn2}) we verify
\begin{eqnarray*}
& & \frac{2 (1 + x^2 y^2)}{(1+ xy)^2} \cdot \frac{x+3}{x-1}
+ cx + 6 \\
& = & 2 \left( 1 - \frac{2z}{(1+ z)^2} \right) \cdot \frac{x+3}{x-1}
+ cx + 6 \\
\left( 2 - \frac{x (x+3)}{x-1} \right) \cdot \frac{x+3}{x-1}
+ cx + 6 \\
& = & 0.
\end{eqnarray*}
Here we used (\ref{lm-2-eqn1}) and (\ref{lm-1-eqn1}).


\end{proof}

Now we will set $t = 4/(1+xy)^2$.  Clearly $t \not =0$.
We next verify that $D = 0$.

By (\ref{lm-3-eqn1}) and (\ref{lm-3-eqn2}) we get
\[\frac{8 y (1 + x^2 y^2)}{(1+ xy)^4} + cx + 6 = 0.\]
Then
\[t^2 y (1 + x^2 y^2) + 2 c x +  3t (1+ xy)^2 =0.\]
Thus
\[D = yt (1 + x^2 y^2) + 3  (1+ xy)^2 + \frac{2 c x}{t} = 0.\]

Next we show that $C = \frac{4 (xy-1)^2}{1-x} \not =0$.

By $D=0$, we have
\[
C = 2 x y^2 \frac{4}{(1+ xy)^2} + 4 (1+ xy)^2 - 4 xy +
[- yt (1 + x^2 y^2) - 3 (1+ xy)^2].
\]
Hence
\begin{eqnarray*}
C &=& \frac{8xy^2}{(1+ xy)^2} + (1+ xy)^2 - 4 xy
- y \frac{4 (1 + x^2 y^2)}{(1+ xy)^2}\\
 &=& \frac{4y}{(1+ xy)^2} \left[ 2xy - 1 - x^2 y^2 \right]
+ (xy-1)^2 \\
 &=& \left( \frac{-4y}{(1+ xy)^2} + 1 \right) (xy-1)^2 \\
 %&=& \left( - {x+3}/(x-1) + 1)...
 &=& \frac{4 (xy-1)^2}{1-x} \not = 0.
\end{eqnarray*}

The next task is to show $B=C$.

We have
\[ C = 4 (xy-1)^2 + x B.\]
Hence
\[ B= \frac{1}{x}
\left[  \frac{4 (xy-1)^2}{1-x} -  4 (xy-1)^2 \right]
= \frac{4 (xy-1)^2}{x} \left[ \frac{1}{1-x} -1 \right] = \frac{4 (xy-1)^2}{1-x}
=C.\]

Finally we verify $A=C$ as well.

\[A = (x^4 y^4 +1) t + x [ C - 2 x y^2 t ]
= C + (x-1)C - 2 x^2 y^2 t + (x^4 y^4 +1) t
= C - 4 (xy-1)^2 + t (x^2 y^2-1)^2
%=C  - 4 (xy-1)^2 + t (xy+1)^2 (xy-1)^2
= C.\]


==> holant-c.tex <==
\section{Remaining Proofs for Pl-Holant$^c$}

\noindent {\bf Proof of Lemma \ref{lemma:interpolate010x}}
%Our start point here is that ${\rm Holant} ([0,1,0,0])$ is \#P-hard.
%This is exactly the perfect matching problem in 3-regular graph
%\cite{DagumL92}. So the problem is \#P-hard if $a=0$.
%
%Now assume that $a \not \in \{-1,0,1\}$, and we use this signature
%to interpolate all the signature of form $[0,1,0,x]$, in particular,
%we can interpolate $[0,1,0,0]$ and finish the hardness reduction.

%\begin{figure}[htbp]
%\begin{center}
%\epsfxsize=4 in \epsffile{gate_Ni.eps} \caption{The recursive
%construction. The signature of every vertex in the gadget is
%$[0,1,0,a]$. } \label{Figure:010x}
%\end{center}
%\end{figure}

The recursive construction is depicted by Figure \ref{Figure:010x}.
By a simple parity argument, every \FF  ~$N_i$ has a signature of
the form $[0,x_i,0,y_i]$. After some calculation, we can get that
they satisfy the following recursive relation:
\[\begin{bmatrix}x_{i+1} \\ y_{i+1} \end{bmatrix}=
\begin{bmatrix}3(a^2+1) & a^3+a \\ 3(a^3+a) & a^6+1 \end{bmatrix}
\begin{bmatrix}x_{i} \\ y_{i} \end{bmatrix}.\]
%%Pinyan: Please double check it.
In this case, the signature we want to interpolate are of arity $3$.
But since all of them are of form $[0,x_i,0,y_i]$ with two
dimensions freedom. We can also use the interpolation method as in
Section \ref{sec:interpolation}. Let $A=\begin{bmatrix}3(a^2+1) &
(a^3+a) \\ 3(a^3+a) & a^6+1
\end{bmatrix}$, then $(A, [1,a]^{\rm T})$ forms a recursive
construction. Since ${\rm det}(A)=3(a^4-1)^2\neq 0$, the first
condition holds. Its characterize equation is $X^2-(a^6+3 a^2+4)X
+3(a^4-1)^2=0$. For this quadratic equation, $\Delta=(a^6-3 a^2
-2)^2+ 12 (a+a^3)^2 >0$. So $A$ has two distinct real eigenvalues.
The sum of the two eigenvalues is $a^6+3 a^2+4$ which is larger than
zero. So they are not opposite to each other. Therefore, the ratio
of these two eigenvalues is not a root of unity and the third
condition holds. Consider the second condition, if the initial
vector $[1,a]$ is a column eigenvectors of $A$. We have
$A\begin{bmatrix}1
\\ a
\end{bmatrix}= \lambda \begin{bmatrix}1 \\ a
\end{bmatrix} $, where $\lambda$ is one eigenvalue of $A$. From
this, we will conclude that $a(a^2-1)(a^4-1)=0$,
%$a^-1=0$
which will not happen given $a \not \in \{-1,0,1\}$. To sum up, this
recursive relation satisfies all the three conditions of Lemma
\ref{lemma:interpolation_conditions} and can be used to interpolate
all the signatures of form $[0,x,0,y]$. This completes the proof.
\qed


The main idea of the proof is to interpolate
all the unary function. If we can do that, we can reduce the problem ${\rm Holant}^* ({\cal
F})$ to ${\rm Holant}^c ({\cal F})$ and finish the proof.
We note that our dichotomy for  ${\rm Holant}^* ({\cal
F})$ also holds for planar structure.
 In some
cases, we can not do that and we prove the theorem separately, mainly using Theorem \ref{thm:a010b}.

\begin{lemma}\label{lemma:interpolation}
If we can construct a gadget with signature $[a,b,c]$, where
$b^2\neq a c$, $b\neq 0$ and $a+c \neq 0$, then we can interpolate
all the unary function. (And hence Theorem \ref{thm:holant-c}
holds.)
\end{lemma}

\begin{proof}
we use the interpolation method as described in Section
\ref{sec:interpolation}. We consider two recursive constructions
$(\begin{bmatrix} a & b \\ b & c \end{bmatrix},
\begin{bmatrix}1 \\ 0 \end{bmatrix} )$ and $(\begin{bmatrix} a & b \\ b & c \end{bmatrix},
\begin{bmatrix}0 \\ 1 \end{bmatrix} )$, and argue that at least one
of them will success given the conditions on $a,b,c$.
We use $A$ to denote $\begin{bmatrix} a & b \\ b & c
\end{bmatrix}$. Since $b^2 \neq ac$, $A$ is non-degenerate,
the first condition of Lemma \ref{lemma:interpolation_conditions} is
satisfied for both of the two recursive constructions. If both
$[1,0]$ and $[0,1]$ are column eigenvectors of $A$, then $b=0$, a
 contradiction. So at least for one of the two recursive constructions,
 the second condition of Lemma \ref{lemma:interpolation_conditions} is satisfied.
 Since $A$ is a real symmetric matrix, so both its eigenvalues are real.
 If the ratio of two real numbers is a root of unity,
 they must be the same or opposite to each other.
 If the two  eigenvalues are the same, we will have $b=0$ and $a=c$,
 a contradiction. If the two eigenvalues are opposite to each other,
 then we have $a+c=0$, also a contradiction.
Therefore, the third condition of Lemma
\ref{lemma:interpolation_conditions} is also satisfied for both of
the two recursive constructions. To sum up, at least one of the two
recursive constructions satisfies all the conditions of Lemma
\ref{lemma:interpolation_conditions}.
  This completes the proof.
\end{proof}

If we can construct a gadget with binary symmetric signature
$[a,b,c]$, which satisfies all the conditions in Lemma
\ref{lemma:interpolation}, then, we are done. Most of the cases, we
prove the theorem by interpolating all the unary signatures.
However, in some cases, we are not able to do that. For example, if
all the signature have the parity condition, then all the unary
signatures we can realize have form $[a,0]$ or $[0,a]$, so we can
not interpolate all the unary signatures. For these cases, our start
point is the Theorem \ref{thm:a010b}.

%Some place we will use the following two lemmas which can be proved from Theorem \ref{thm:a010b}.
%
%\begin{lemma} \label{thm:a000b-and-010x}
%Let $ab=\neq 0$ and $x\neq \pm 1$. Then Pl-Holant$^c(\{[a,0,0,0,b],[0,1,0,x]\})$ is \#P-hard.
%\end{lemma}
%\begin{proof}
%\end{proof}


We define some families of symmetric signatures, which will be used
in our proof.
\begin{eqnarray*}
{\cal G}_1&=&\{[a,0,0,\cdots,0,b] |ab \neq 0 \}\\
{\cal G}_2&=&\{[x_0,x_1,\cdots,x_k] | \forall i \mbox{ is even}, x_i=0 \mbox{ or } \forall i \mbox{ is odd}, x_i=0  \}\\
{\cal G}_3&=&\{[x_0,x_1,\cdots,x_k] | \forall i, x_i+x_{i+2}=0  \}\\
{\cal M} &=&\{f | f \mbox{is realizable by some matchgate.} \}
\end{eqnarray*}
We note that ${\cal G}_1$, ${\cal G}_2$ and ${\cal G}_3$ are
supersets of ${\cal F}_1$, ${\cal F}_2$ and ${\cal F}_3$
respectively. And we further have ${\cal F}_2 \subseteq {\cal M} \subseteq {\cal G}_2$ The following several lemmas all have the form ``If
${\cal F} \not \subseteq {\cal A}$, then Theorem \ref{thm:holant-c}
holds." After proving that, in the later lemma, we only need to
consider the case that ${\cal F} \subseteq {\cal A}$.

\begin{lemma}\label{lemma:inG1G2G3}
If ${\cal F} \not \subseteq {\cal G}_1 \cup {\cal G}_2\cup {\cal
G}_3$, then Theorem \ref{thm:holant-c} holds.
\end{lemma}

\begin{proof}
Since ${\cal F} \not \subseteq {\cal G}_1 \cup {\cal G}_2\cup {\cal
G}_3$, there exists a $f \in {\cal F}$ and  $f \not \in {\cal G}_1
\cup {\cal G}_2\cup {\cal G}_3$. Since all the unary signatures are
in ${\cal G}_3$, the arity of $f$ is larger than $1$ and $f$ is
non-degenerate. There are two cases according to whether $f$ has a
zero entry or not.

(1) $f$ has some zero entries. If there exists a sub signature of
$f$ has the form $[0,a,b]$ or $[a,b,0]$, where $ab\neq 0$, then we
are done by Lemma \ref{lemma:interpolation}. Otherwise, we can
conclude that there is no two successive non-zero entries. So the
signature $f$ is like this $[0^{i_0}x_1 0^{i_1} x_2 0^{i_2}\cdots
x_k 0^{i_k}] $, where $x_j \neq 0$ and for all $1\leq j \leq k-1$,
$i_j\geq 1$. If for all $1\leq j \leq k-1$, $i_j $ is odd, then
$f\in {\cal G}_2$, a contradiction. Otherwise there exists a sub
signature of form $[x,0,0,\cdots, 0 ,y]$, where $xy\neq 0$ and there
are even number of $0$s between $x$ and $y$. If this is the whole
$f$, then $f\in {\cal G}_1$, a contradiction. So there is one $0$
before $x$ or after $y$. By symmetric, we assume there is a $0$
before $x$, so we have a sub signature $[0,x,0,0,\cdots, 0 ,y]$,
whose arity is even and larger than $3$. We call its dangling edges
$1,2, \cdots, 2k$. Then for every $i=1,2,\cdots, k-1$, we connect
dangling edges $2i+1$ and $2i+2$ together to a regular edge. After
that, we have a \FF ~with arity 2, and its signature is $[0,x,y]$.
Then we are done by Lemma \ref{lemma:interpolation}.

(2) $f$ has no zero entry. We only need to prove that we can
construct a function $[a',b',c']$ satisfying the three conditions in
Lemma \ref{lemma:interpolation}. Suppose all sub signatures of $f$
with arity 2 do not satisfy all the three conditions. For each
sub-signature $[a',b',c']$, either $a'+c'=0$, or $b'^2=a'c'$. If all
of them satisfy $a'+c'=0$, then $f \in \mathcal{G}_3$. A
contradiction. If all of them satisfy  $b'^2=a'c'$, then $f$ is
degenerate. A contradiction. W.l.o.g, we can assume there is a
sub-signature $[a,b,c,d]$ of $f$, such that $a+c=0$, $b+d \neq 0$,
and $c^2=bd$. Combining two $[a,b,c,d]$, we can get a function
$[a',b',c']=[a^2+2b^2+c^2,ab+2bc+cd,b^2+2c^2+d^2]$. $b'=c(b+d) \neq
0$. $a'+c'=a^2+3b^2+3c^2+d^2>0$. Because $c^2=bd$,
$a'c'-b'^2=a^2b^2+2a^2c^2+a^2d^2+2b^4+4b^2c^2+2b^2d^2\neq 0$. We are
done by Lemma \ref{lemma:interpolation}.
\end{proof}

The following lemmas are proved in the main text.

\begin{lemma}\label{lemma:inG1MG3}
If ${\cal F} \not \subseteq {\cal G}_1 \cup {\cal M} \cup {\cal
G}_3$, then Theorem \ref{thm:holant-c} holds.
\end{lemma}


\begin{lemma}\label{lemma:010x}
If $[0,1,0,x] \in {\cal F}$ (or $[0,1,0,x]\in {\cal F}$) where $x\neq \pm 1$, then Theorem \ref{thm:holant-c} holds.
\end{lemma}

The following is the remaining proof of the dichotomy for Pl-Holant$^c$

\begin{lemma}\label{lemma:inG1F2G3}
If ${\cal F} \not \subseteq {\cal G}_1 \cup {\cal F}_2\cup {\cal
G}_3$, then Theorem \ref{thm:holant-c} holds.
\end{lemma}

\begin{proof}
If ${\cal F} \not \subseteq {\cal G}_1 \cup {\cal G}_2\cup {\cal
G}_3$, then by Lemma \ref{lemma:inG1G2G3}, we are done. Otherwise,
there exists a signature $f \in {\cal F} \subseteq {\cal G}_1 \cup
{\cal G}_2\cup {\cal G}_3 $ and $f \not \in {\cal G}_1 \cup {\cal
F}_2\cup {\cal G}_3$. Then it must be the case that $f \in {\cal
G}_2$. Note that every signature with arity less than $3$ in ${\cal
G}_2$ is also contained in ${\cal G}_1 \cup  {\cal G}_3$, so $f$ is
of arity larger than $2$. Since $f \not \in {\cal G}_1$, there is
some non-zero in the middle of the signature $f$, after
normalization, we can assume there is a sub signature of form
$[0,1,0,x]$ (or $[x,0,1,0]$). If $x\neq \pm 1$, then by Lemma
\ref{lemma:010x}, we are done.
Otherwise, for every such pattern , we have $x=\pm 1$. Since $f \not
\in {\cal F}_2$, then there is some sub signature $[0,1,0,-1]$ and
because $f \not \in {\cal G}_3$, there is some sub signature
$[0,1,0,1]$. Therefore, there is a sub signature $[1,0,1,0,-1]$ of
$f$. Then by Lemma \ref{thm:a010b}, we
know that the problem is \#P-hard and we are done. This completes
the proof.
\end{proof}

\begin{lemma}\label{lemma:inG1G3}
If ${\cal F} \not \subseteq {\cal G}_1 \cup  {\cal G}_3$, then
Theorem \ref{thm:holant-c} holds.
\end{lemma}

\begin{proof}
If ${\cal F} \not \subseteq {\cal G}_1 \cup {\cal F}_2\cup {\cal
G}_3$, then by Lemma \ref{lemma:inG1F2G3}, we are done. Otherwise,
there exists a signature $f \in {\cal F} \subseteq {\cal G}_1 \cup
{\cal F}_2\cup {\cal G}_3 $ and $f \not \in {\cal G}_1 \cup {\cal
G}_3$. Then it must be the case that $f \in {\cal F}_2$. Note that
every signature with arity less than $3$ in ${\cal F}_2$ is also
contained in ${\cal G}_1 \cup  {\cal G}_3$, so $f$ is of arity
larger than $2$. Then $f$ has a sub signature $[1,0,1,0]$ or
$[0,1,0,1]$. By symmetry, we assume it is $[1,0,1,0]$. If ${\cal F}
\subseteq {\cal F}_1 \cup {\cal F}_2 \cup {\cal F}_3 $, then Theorem
\ref{thm:holant-c} trivially holds and there is nothing to prove. If
not, there exists a signature $g$ is in ${\cal G}_1-{\cal F}_1 \cup
{\cal F}_2 \cup {\cal F}_3 ~(\subseteq{\cal G}_1-{\cal F}_1)$ or
${\cal G}_3-{\cal F}_1 \cup {\cal F}_2 \cup {\cal F}_3
~(\subseteq{\cal G}_3-{\cal F}_3)$.

For the first case,  $g \in ({\cal G}_1-{\cal F}_1)$, then after a
scale, $g$ is of form $[1,0,0,\cdots, b]$, where $b \not \in
\{-1,0,1\}$. If the arity of $g$ is odd, we can realize $[1,b]$. (We
connect its every two dangling edges into one edge and left one
dangling edge.) Then connecting this unary signature to one dangling
edge of $[1,0,1,0]$,
 we can realize a binary
signature $[1,b,1]$.
% by a ${\cal F}$-gate as in Fig \ref{}.
Then by Lemma \ref{lemma:interpolation}, Theorem \ref{thm:holant-c}
holds. If the arity of $g$ is even, we can realize $[1,0,b]$ (left
two dangling edges). By connecting  one of its dangling edge to one
dangling edge of $[1,0,1,0]$, we can have a new ternary signature
$[1,0,b,0]$.
% by a ${\cal F}$-gate as in Fig \ref{}.
By lemma \ref{lemma:010x}, we are done.

For the second case $g \in ({\cal G}_3-{\cal F}_3)$, then $g$ has a
sub signature of form $[1,b]$, where $b \not \in \{-1,0,1\}$. By the
same argument as above, Theorem \ref{thm:holant-c} holds. This
completes the proof.
\end{proof}


\begin{lemma}\label{lemma:inG1F3}
If ${\cal F} \not \subseteq {\cal G}_1 \cup  {\cal F}_3$, then
Theorem \ref{thm:holant-c} holds.
\end{lemma}

\begin{proof}
If ${\cal F} \not \subseteq {\cal G}_1 \cup {\cal G}_3$, then by
Lemma \ref{lemma:inG1G3}, we are done. Otherwise, there exists a
signature $f \in {\cal F} \subseteq {\cal G}_1 \cup {\cal G}_3 $ and
$f \not \in {\cal G}_1 \cup {\cal F}_3$. Then it must be the case
that $f \in {\cal G}_3$ , and $f$ has a sub signature of form
$[1,a,-1]$, where $a \not \in \{-1,0,1\}$.
%XMJ: the length of this sub-signature is 3,
%because all signatures of length 2 are in G_1.
%because $f \not \in {\cal F}_3$, $a \not \in \{-1,0,1\}$.

If ${\cal F}  \subseteq (\{[1,0,1] \} \cup  {\cal G}_3)$, then ${\rm
Holant}^* ({\cal F})$  is polynomial time computable by Theorem
\ref{thm:main} and as a result Theorem \ref{thm:holant-c} trivially
holds and there is nothing to prove.

If not, there exists a signature $g \in {\cal F}  \subseteq {\cal
G}_1 \cup  {\cal G}_3$ and $g \not \in \{[1,0,1] \} \cup  {\cal
G}_3$. Then it mush be the case that $g \in {\cal G}_1$. The arity
of $g$ is large than $1$. %,because G_3 contains all functions of arity 1.

%\begin{figure}[htbp]
%\begin{center}
%\epsfxsize=2 in \epsffile{gata_for_lemma2.6.eps} \caption{The
%function on degree 2 nodes is $[1,a,-1]$, and the function on degree
%3 nodes is $[1,0,0,b]$. } \label{Figure:[1,a^2b,b^2]}
%\end{center}
%\end{figure}



If the arity of $g$ is $2$, then $g$ is of form $[1,0,b]$, where $b
\not \in \{-1,0,1\}$. Connecting two signatures $[1,0,b]$ to the
both sides of one binary signature $[1,a,-1]$, we can get a new
binary signature $[1,ab, -b^2]$. It satisfies all the conditions of
Lemma \ref{lemma:interpolation}, and we are done. If the arity of
$g$ is larger than $2$, then we can always realize a signature
$[1,0,0,b]$, where $b\neq 0$. (We connect the unary signature
$[1,a]$ to all its dangling edges except the three ones.)
 Then we can use an \FF ~as Figure \ref{Figure:[1,a^2b,b^2]}.
Its signature is $[1,a^2b, b^2]$, and by Lemma
\ref{lemma:interpolation}, we are done. This completes the proof.
\end{proof}



By the above lemmas, the only case we have to handle is that ${\cal
F} \subseteq {\cal G}_1 \cup  {\cal F}_3$. This is done by the
following lemma. which completes the proof of Theorem
\ref{thm:holant-c}.

\begin{lemma}\label{lemma:G1F3}
If ${\cal F}  \subseteq {\cal G}_1 \cup  {\cal F}_3$, then Theorem
\ref{thm:holant-c} holds.
\end{lemma}

\begin{proof}
If ${\cal F} \subseteq {\cal F}_1 \cup {\cal F}_3$ or ${\cal
F}\subseteq {\cal U} \cup {\cal F}_3 \cup \{[1,0,1]\}$, then ${\rm
Holant}^c({\cal F})$ is computable in polynomial time and
Theorem\ref{thm:holant-c} holds. Otherwise, there are two cases.
There exists $f\in {\cal F} $ such that $f \in {\cal G}_1$ but $f
\not \in{\cal F}_1 \cup {\cal U} \cup {\cal F}_3 $. So the arity of
$f$ is larger than $1$. W.l.o.g, we can assume $f$ has form
$[1,0,a]$ or $[1,0,0,a]$, where $a \not \in \{-1,0,1\}$. (By
connecting its dangling edges together except two or three depends
on the parity of the arity of $f$. ) The other case is that there
exists $f_1, f_2\in {\cal G}_1$ such that $f_1 \in {\cal F}_1$ but
$f_1 \not \in{\cal U} \cup {\cal F}_3 \cup \{[1,0,1]\}$, and $f_2
\in {\cal U}$ but $f_2 \not \in {\cal F}_1$. So the arity of $f_1$
is larger than $2$ and with form $[1,0,0,\cdots,\pm 1]$, and $f_2$
is of form $[1,a']$, where $a' \not \in \{-1,0,1\}$. By connecting
all the dangling edges of $f_1$ except two with $f_2$, we can
construct a \FF ~with signature of form $[1,0,a]$, where $a \not \in
\{-1,0,1\}$.This is one of the above two forms.

If ${\cal F}  \subseteq {\cal G}_1 \cup  \{[0,1,0]\}$, then
 ${\rm Holant}^c
({\cal F})$ is computable in polynomial time and Theorem
\ref{thm:holant-c} holds. Otherwise, there exists $g\in {\cal F}
\subseteq {\cal G}_1 \cup  {\cal F}_3 $, and $g \not \in {\cal G}_1
\cup  \{[0,1,0]\}$. Then $g$ must have one of the following sub
signatures: $[1,1,-1],[1,-1,-1],[1,0,-1,0],[0,1,0,-1]$. By
symmetric, we only need to consider two cases $[1,1,-1]$ and
$[1,0,-1,0]$.
%Right. When "symmetric", f=[1,0,a], will turn into [a,0,1]=a[1,0,1/a], 1/a \not \in \{-1,0,1\} either.

According to $f$ and $g$, we have four cases. If $f=[1,0,a]$ and
$g=[1,1,-1]$, then connecting them together into a chain $fgf$, we
can realize $[1,a,-a^2]$. By Lemma \ref{lemma:interpolation}, we are
done. If $f=[1,0,a]$ and $g=[1,0,-1,0]$, for each of dangling edges
of $g$, we extend it by one copy of $f$. Then we can realize
$[1,0,-a^2,0]$. So by lemma \ref{lemma:010x}, we are done. If $f=[1,0,0, a]$ and $g=[1,1,-1]$, we can connect a unary
signature $[1,1]$ (sub signature of $g$) to one dangling edge of
$f$, and realize a binary signature $f=[1,0,a]$. This reduce to the
first case, which has been proved. If $f=[1,0,0,a]$ and
$g=[1,0,-1,0]$, we can realize a unary signature $[1,a]$ from $f$
and then connect this unary signature to one dangling edge of $g$ to
realize $[1,-a,-1]$. Note that $[1,-a,-1]\not \in {\cal G}_1 \cup
{\cal F}_3$, by Lemma \ref{lemma:inG1F3}, we are done.
\end{proof}




==> lemma001.tex <==
\section{Proof of Lemma \ref{lemma001}}
\begin{lemma}
Pl-Holant$(\mathcal{F}\cup \{[0,0,1],[1,0], [1,0,1], [1,0,1,0],[1,0,1,0,1] \cdots\})$ is \#P-hard (or in P), iff Pl-Holant$^c(\mathcal{F}\cup \{[0,0,1], [1,0,1], [1,0,1,0],[1,0,1,0,1] \cdots\})$  is \#P-hard (or in P).
\end{lemma}


\begin{proof}
There is one more function $[1,0]$ in the second problem than the first problem, so obviously, the first one can be reduced to the second one.

Now, we show the reduction in the other direction also holds. By the proof in this paper and \cite, when the second problem is proved to be \#P-hard, either $\#[1,0,0,1]|[1,1,0]$ or  $\#[1,1,0,0]|[1,0,1]$ is reduced to it by a chain of reductions. There are only three reduction methods in this reduction chain, direct gadget construction, polynomial interpolation, and holographic reduction.

Given an instance $G$ of $\#[1,0,0,1]|[1,1,0]$ or $\#[1,1,0,0]|[1,0,1]$, we consider graph $G\cup G$, which denotes the graph composed of two $G$.

Notice the value of $\#[1,0,0,1]|[1,1,0]$ or $\#[1,1,0,0]|[1,0,1]$ on the instance $G$ is  positive, so we can get it from its square, the value of instance $G\cup G$. Suppose the instance $G$ is reduced to instances $G_1,G_2,\ldots G_m$ of the second problem in this finite reduction chain. By the same reduction, if we start from $G \cup G$, we get instances of this form $G_1 \cup ,G_2 \cup G_2,\ldots G_m' \cup G_m'$. (We many reduce $G \cup G$ to more instances than $G$, because when using polynomial reduction, instance of larger size may reduced to more graphs.)

%By the same reduction proof, we can get the value of  $G \cup G$.


Now we only need to show how to get the value of  instances $G_1 \cup ,G_2 \cup G_2,\ldots G_m' \cup G_m'$ in the first problem. $G_i \cup G_i$ is a planar graph with some degree one vertices associated with function $[0,1]$. We want to replace each pair of functions $[0,1]$ by $[0,0,1]$ keeping planarity.

Take a spanning tree of the dual graph of $G_i$. Let the outer face is the root. Choose an arbitrary leaf of this tree, which corresponds to a face $C$ of $G_i$. Suppose $C'$ is the face corresponds to the father of $C$ in the tree. If there are even many degree one vertices with function $[0,1]$ in face $C$, we can perfectly match them and realize them using $[0,0,1]$ keeping planarity in this face. If there are odd many, we choose one edge $[1,0,1]$ on the boundary between $C$ and $C'$, and add a vertex $[1,0,1,0,1]$ connected by two vertices $[0,1]$ on this edge, which is a simple gadget has the same function as $[1,0,1]$. We put one vertex $[0,1]$ in face $C$, and the other one in face $C'$. Now, there are even many  $[1,0,1]$ in $C$. We handle them as the first case. Repeating this process, until only root is left. Do the same thing for the two $G_i$ in $G_i \cup G_i$, and at last perfectly math the $[0,1]$ vertices in the two outer faces and realize them by $[0,0,1]$. We get an instance of the first problem, which has the same value.
\end{proof}

